Understanding Local Robustness of Deep Neural Networks under Natural Variations

Deep Neural Networks (DNNs) are being deployed in a wide range of settings today, from safety-critical applications like autonomous driving to commercial applications involving image classifications. However, recent research has shown that DNNs can be brittle to even slight variations of the input data. Therefore, rigorous testing of DNNs has gained widespread attention. While DNN robustness under norm-bound perturbation got significant attention over the past few years, our knowledge is still limited when natural variants of the input images come. These natural variants, e.g. a rotated or a rainy version of the original input, are especially concerning as they can occur naturally in the field without any active adversary and may lead to undesirable consequences. Thus, it is important to identify the inputs whose small variations may lead to erroneous DNN behaviors. The very few studies that looked at DNN's robustness under natural variants, however, focus on estimating the overall robustness of DNNs across all the test data rather than localizing such error-producing points. This work aims to bridge this gap. To this end, we study the local per-input robustness properties of the DNNs and leverage those properties to build a white-box (DeepRobust-W) and a black-box (DeepRobust-B) tool to automatically identify the non-robust points. Our evaluation of these methods on three DNN models spanning three widely used image classification datasets shows that they are effective in flagging points of poor robustness. In particular, DeepRobust-W and DeepRobust-B are able to achieve an F1 score of up to 91.4% and 99.1%, respectively. We further show that DeepRobust-W can be applied to a regression problem in another domain. Our evaluation on three self-driving car models demonstrates that DeepRobust-W is effective in identifying points of poor robustness with F1 score up to 78.9%.

==> Makefile <==
# $Id: Makefile 1833 2006-06-19 21:51:36Z witchel $

.SUFFIXES: .fig .dvi .ps .pdf

VERSION = 0.0

#----------------------------------------------------------------------
# Source files.  Edit these variables for each new paper.
#----------------------------------------------------------------------

name = main_issta

all: pdf bib

#----------------------------------------------------------------------
# LaTeX commands.
#----------------------------------------------------------------------

%.dvi:%.tex
	pdflatex $<

dvi: $(name).tex *.tex
	pdflatex $<

rub: $(name).tex 
	rubber -Wrefs -Wmisc $(name)

twice:
	pdflatex $(name)
	pdflatex $(name)

bib:
	bibtex $(name)
	pdflatex $(name)
	pdflatex $(name)


latex_junk = 	$(name).dvi \
		*.aux \
		*.log \
		$(name).blg \
		$(name).toc \
		$(name).out \
		psfig.aux \
		*.bbl \
		*.pdfsync \
		*.fdb_latexmk \
		*.fls \
		*.synctex.gz


#----------------------------------------------------------------------
# Postscript/PDF generation.
#----------------------------------------------------------------------

$(name).ps:
ps: $(name).dvi *.tex
	latex $(name).tex && latex $(name).tex
	$(DVIPS) -P pdf -t letter -o $(name).ps $(name).dvi

summary: summary.dvi

#DVIPS = dvips
DVIPS = dvips

%.ps:%.dvi
	$(DVIPS) -P pdf -t letter -o $@ $<

%.ps2:%.dvi
	$(DVIPS) -t letter -o ps2.tmp -p 2 $<
	mpage -2 -P ps2.tmp > $@
	rm ps2.tmp

pdf: 
	pdflatex $(name).tex

# DISTILL = distill
DISTILL_FLAGS = -embedallfonts on -maxsubsetpct 100

DISTILL = ps2pdf
#DISTILL_FLAGS =

%.pdf:%.ps
	$(DISTILL) $(DISTILL_FLAGS) $<

#----------------------------------------------------------------------
# Document previewers.
#----------------------------------------------------------------------

x:
	xdvi -s 5 $(name) &

gv: $(name).ps
	ghostview $(name).ps &


# Garbage files.
junk = $(latex_junk) *.ps *.pdf *.out


#----------------------------------------------------------------------
# Miscellaneous.
#----------------------------------------------------------------------

tags:
	etags $(latex_files)

clean:
	rm -f $(junk)

count:
	wc $(latex_files)


==> abstract.tex <==
\begin{abstract}
Deep neural networks(DNNs) are being deployed in a wide range of settings today, from commercial applications such as language translation and retail, to safety-critical domains such as medical diagnosis and autonomous driving. However, recent research has shown that DNNs can be brittle to even slight variations in their input data. Therefore, rigorous testing and analysis of the robustness of DNNs has gained widespread attention. However, existing work on the robustness of DNNs either focuses on  robustness of DNNs to adversarial examples, which are artificial, and/or supports the development phase of DNNs with testing and re-training them.

In this work, we study the robustness of DNNs for image recognition tasks under natural variations of the input data. In particular, we study robustness under spatial variations, such as rotation and translation of images. We adopt a point-wise robustness measure called neighbor accuracy and classify each data point in the input space as either strong or weak depending on its high or low neighbor accuracy respectively. We observe that weak data points are shared across models, and tend to be located towards the class boundaries in the feature space. Furthermore, a point's neighbor accuracy is highly correlated with the diversity of a model's prediction on the point's neighbor points. We leverage these observations to design two analyses that can provide real-time feedback to the end-user, on the robustness of the DNN in the vicinity of the current input. Our evaluation of these analyses on nine DNN models spanning three widely used image classification datasets, shows that they are effective in flagging points of poor robustness. % evaluate with several state-of-the-art models for three widely used image classification datasets. Our evaluation results show that DeepRobust is able to achieve a precision up to 98.6\% and a recall up to 96.7\% for these dataset. 
% We also show that our results are generalizable to not only image classification tasks but also to face recognition tasks.
\cmt{We could replace the qualitative performance statements above with quantitative measures when the final results are in.}

\keywords{Deep Neural Networks \and Software Testing}
\end{abstract}

==> into_back.tex <==
%auto-ignore
\section{Introduction}\label{sec:intro}

%%%Background: Rise of DL and connection to SE
Deep Neural Networks (DNNs) have achieved an unprecedented level of performance over the last decade in many sophisticated areas such as image recognition~\cite{krizhevsky2012imagenet}, self-driving cars~\cite{bojarski2016end} and playing complex games~\cite{44806}. These advances have motivated Information Technology companies to integrate AI capabilities into software and services, and to adapt their software development flows to incorporate AI software components~\cite{MSR-ICSE-SEIP.2019}. This trend has, in turn, spawned a new area of research within software engineering addressing the quality assurance of DNN components~\cite{pei2017deepxplore,tian2017deeptest,zhang2018deeproad, ma2018mode, kim2019guiding, CRADLE:ICSE2019, DeepStellar:FSE2019, Islam:FSE2019, Li:FSE2019, Apricot:ASE2019, tian2019deepinspect, Sensei:ICSE2020}. 
%\mukul{Add remaining references from ICSE2019, FSE2019, ASE2019.} 

%%%Background: Importance of robustness testing
Notwithstsanding the impressive capabilities of DNNs, recent research has shown that DNNs can be easily fooled, \ie made to mispredict, with a little variation of the input data~\cite{goodfellow2014explaining,engstrom2019exploring,tian2017deeptest}. For example,  a large body of work showed that image variants \emph{artificially} created by adding a small pixel-level perturbation into the original input can easily fool a DNN into misclassification~\cite{szegedy2013intriguing,goodfellow2014explaining,carlini2017towards}. More recent work has also shown that \emph{natural} variants of input data, \eg rotating an image, changing the lighting conditions, \etc can also make a DNN mispredict~\cite{engstrom2019exploring, pei2017deepxplore}. 
As the name suggests, these variations %may be perceivable by a human but 
can occur naturally in the field without any active adversary. %\cmt{IMHO perhaps the contrast with \emph{adversarial variants} is that these variations occur \emph{naturally in the field}, without any active adversary. The fact that they are perceivable may not be relevant, or in fact even true. I mean an observer (in the field) may not detect a natural variation as a change since they do not have a reference instance to compare against.}
Such natural variants may lead to serious consequences for safety-critical applications such as self-driving cars~\cite{tian2017deeptest,zhang2018deeproad}, medical diagnosis, \etc 
Thus, understanding, testing, and analyzing the robustness properties of these variants is important. 


However, our knowledge of DNN robustness under such natural variations is limited. For instance,  some works improve a DNN's robustness against natural variants generated by spatially transformed images using data augmentation~\cite{engstrom2019exploring} and extra regularization term~\cite{trade_alp_spatial}. Balunovic~\etal~\cite{geometric_certify} provide a DNN verification method for spatial transformation. However, these works focus on analyzing the overall robustness of the DNN rather than trying to pinpoint the images that may have robustness issues. From a traditional software engineering point of view, this is analogous to saying this software has bugs without localizing the bugs. Our current work focuses on localizing such {\em weak points} that pose significant threats to a DNN model's robustness. 

%However, our knowledge of DNN robustness under such natural variations is limited. For instance,  some works improve a DNN's robustness against natural variants generated by spatially transformed images using data augmentation~\cite{engstrom2019exploring} and extra regularization term~\cite{trade_alp_spatial}. Balunovic~\etal~\cite{geometric_certify} provide a DNN verification method for spatial transformation. However, we still do not have a clear understanding of the circumstances in which robustness issues arise, or questions about whether robustness problems are inherent to a dataset or depend on the model, etc.
%idea about the robustness properties of DNN against these transformations: for example, in which cases the DNNs are more prone to failure, whether robustness is inherent to the dataset or depends on the model, etc.

To bridge this gap, in this paper, we first quantify the robustness property of DNN per input data point by considering a population of natural variants of the point and measuring the fraction of this population classified correctly by the DNN - a high fraction of correct classifications indicates good robustness and vice versa. We term this measure {\em neighbor accuracy}. \edited{It is based on an intuitive point-wise version of spatial robustness commonly used by existing literatures \cite{engstrom2019exploring, engstrom2017rotation, spatial2018}.} We then conduct an in-depth study of different robustness properties of DNNs with respect to ~{\em natural} variants based on \edited{the neighbor accuracy measurement}. Given that the number of natural neighbor of an image can be infinite we focus our study to the variants generated by spatial transformations, viz., rotation, and translation, following the previous work~\cite{engstrom2019exploring,trade_alp_spatial,geometric_certify}.
We also focus on robustness analysis of individual input as opposed to estimating overall robustness of a model across all the test data~\cite{pei2017deepxplore, tian2017deeptest, zhang2018deeproad,goodfellow2014explaining, carlini2017towards} as done by prior work, as 
% While studying the robustness of a model, most existing studies evaluate the accuracy of a DNN model on naturally or adversarially generated image variants~\cite{pei2017deepxplore, tian2017deeptest, zhang2018deeproad,goodfellow2014explaining, carlini2017towards} and report overall robustness of the model under test. 
not all the input images in a dataset are equally likely to fail. \edited{Some data points are much weaker than other data points with respect to robustness.} For example, consider~\Cref{fig:motivation_different_classes}: although the original bird image (a) is predicted correctly by a DNN, its different rotated variations in Figures (b)-(d) are mispredicted to three different classes. In contrast, another bird image and its rotated versions, shown in Figure~\ref{fig:motivation_different_classes} (e)-(h), are correctly classified by the same DNN under the same degrees of rotation. 
We call such per data point robustness as local robustness. \edited{ \Cref{fig:neighbor_acc_3dtsne} further shows a t-SNE \cite{vanDerMaaten2008} (x,y axes) and neighbor accuracy (z axis) visualization of the testing set of the self-driving car dataset when using~epoch \cite{epoch} and the ~\cifar~dataset when using~\resnet \cite{he2016deep}, respectively. The lower (i.e. the smaller the neighbor accuracy) a point is, the more non-robust it is according to our definition. Though the two datasets have completely different distributions of local robustness landscape. They both have points having different degrees of local robustness.}

It is important to understand such local robustness properties, \ie how
the weak points differ characteristically from their robust counterparts.  \edited{Such knowledge can be useful to estimate how much we can trust a DNN's prediction on the natural variation of the current input.} 

%  Such knowledge can be useful to estimate how muchwe can rely on a DNN predicted result\textemdash users are likely to trust {\em less} if they know in advance the input image lies in a non-robust region. 

% \todo{Ziyuan: I feel this sentence is confusing.}

\begin{figure}[t]
\centering
    \subfloat[\ang{0},bird\label{fig:bird1}]
    {\includegraphics[width=0.11\textwidth]{{"figure/674_0_2"}.png}}
    \hspace{0.01\textwidth}%
    \subfloat[+\ang{6},airplane]
    {\includegraphics[width=0.11\textwidth]{{"figure/20674_2_0"}.png}}
    \hspace{0.01\textwidth}%
    \subfloat[+\ang{24},cat]
    {\includegraphics[width=0.11\textwidth]{{"figure/80674_8_3"}.png}}
    \hspace{0.01\textwidth}%
    \subfloat[-\ang{9},dog]
    {\includegraphics[width=0.11\textwidth]{{"figure/130674_13_5"}.png}}
    
    \subfloat[\ang{0},bird\label{fig:bird2}]
    {\includegraphics[width=0.11\textwidth]{{"figure/75_0_2"}.png}}
    \hspace{0.01\textwidth}%
    \subfloat[+\ang{6},bird]
    {\includegraphics[width=0.11\textwidth]{{"figure/20075_2_2"}.png}}
    \hspace{0.01\textwidth}%
    \subfloat[+\ang{24},bird]
    {\includegraphics[width=0.11\textwidth]{{"figure/80075_8_2"}.png}}
    \hspace{0.01\textwidth}%
    \subfloat[-\ang{9},bird]
    {\includegraphics[width=0.11\textwidth]{{"figure/130075_13_2"}.png}}
\caption{\textbf{\small{A well-trained standard resnet model~\cite{engstrom2019exploring} misclassifies the rotated variations of a bird image into three different classes, although the original un-rotated image is classified correctly. 
\textbf{(Bottom row)} The same model successfully classifies all the rotated variants of another bird image taken from the same test dataset. The sub-captions consist of rotation degrees, and the predicted classes.}}}
\label{fig:motivation_different_classes}
\vspace{-5mm}
\end{figure} 


\begin{figure}[t]
\centering
    \subfloat[\sdc]
    {\includegraphics[width=0.22\textwidth]{{"figure/tsne/self_driving_epoch"}.pdf}}
    \hspace{0.01\textwidth}%
    \subfloat[\cifar]
    {\includegraphics[width=0.22\textwidth]{{"figure/tsne/cifar10_resnet"}.pdf}}
    \hspace{0.01\textwidth}%

\caption{\textbf{\small{t-SNE visualization of neighbor accuracy of sampled 1000 points whose original images are correctly classified. The x, y axes are from t-SNE and the z axis (and the color bar) is the neighbor accuracy.\ziyuan{explain what you are getting from this figure.}}}}
\label{fig:neighbor_acc_3dtsne}
\vspace{-5mm}
\end{figure} 


To this end, we conduct a detailed empirical analysis of the robustness properties per input image and use the data-driven knowledge to build tools that can automatically detect the non-robust inputs both in white-box and black-box settings. 
Our analysis with three well-known object recognition datasets across three popular DNN models, \ie a total of nine DNN-dataset combinations, reveal several interesting properties of local robustness of a DNN \wrt natural variants:

\begin{itemize}[leftmargin=*]
\item For each DNN, some inputs are more robust than others and most of the robust points remain robust across all the models and vice versa, \ie robustness properties are intrinsic to the dataset rather than the DNN (RQ1). 
\item The weak points are concentrated near the class decision boundaries of the DNN in the feature space (RQ2a).
\item The variants of weaker points show more output diversity, \ie they tend to be misclassified to many different classes (RQ2b). 
%, \ie the degree of robustness is strongly correlated with the number of different classes that different variants of a point get classified to. ~\todo{will polish this}
\end{itemize}

Based on these findings, we develop two techniques that can identify points of poor robustness at runtime, thereby providing a means of, input-specific, real-time feedback about robustness to the end-user.
Our white-box and black-box detectors can identify weak, \aka non-robust, points with precision 89.8\% and 99.2\%, and recall 95.8\% and 99.0\%, respectively, at neighbour accuracy cutoff 0.75.

%%% Contributions
In summary, we make the following contributions: 
\begin{itemize}[leftmargin=*]
    \item \textbf{Empirical study \& metric:} We conduct an empirical study of robustness properties of DNNs to natural variations, using nine DNN models, spanning three popular image classification datasets. We adopt a metric called neighbor accuracy to quantify the robustness of the DNN for any given point in the DNN input space.
    \item \textbf{Characterization of robustness:} We identify three key properties to characterize DNN robustness, namely, the distribution of points of weak robustness, the spatial distribution of these weak points in the DNN's representation space, these weak points across different DNNs on the same dataset, and the diversity in the (incorrect) classifications of natural variants of a data point. Our study reveals interesting findings for these properties.
    \item \textbf{Detection of weak points:} Leveraging the above properties, we develop two different methods: a white-box (\toolWB) and a black-box (\toolBB), to automatically detect weak points in real-time. \edited{We evaluate both methods on nine DNN models spanning three image classification datasets and further evaluate \toolWB on three DNN models on a self-driving car dataset.}
    %provide input-specific real-time feedback to the end-user on the robustness of DNN in the vicinity of a given input.
\end{itemize}


% Notwithstsanding the impressive capabilities of DNNs, recent research has shown that a DNN can be easily fooled, \ie made to mispredict, with a little variation of the input data~\cite{goodfellow2014explaining,engstrom2019exploring,tian2017deeptest}. This may lead to serious consequences for safety-critical applications such as self-driving cars, medical diagnosis, \etc 
% As a result, understanding, testing, and analyzing the robustness properties of DNNs have attracted significant attention in recent years. 


% %% Problem specification
% Much of the existing work on robustness of DNNs has focused on adversarial instances -- imperceptible variants of natural DNN inputs, \emph{artificially} created by adding a small amount of noise into the original input so as to fool the DNN into misclassification~\cite{szegedy2013intriguing,goodfellow2014explaining,carlini2017towards}. 
% %This includes different techniques to generate adversarial examples~\cite{goodfellow2014explaining, carlini2017towards}, to automatically distinguish adversarially modified inputs from natural ones~\cite{feinman2017detecting,metzen2017detecting}, to verify the robustness of DNNs to adversarial inputs ~\cite{wang2018formal, Wang:2018:EFS:3327345.3327533, wang2018mixtrain}, techniques to harden DNNs against adversarial attack ~\cite{gu2014towards,shaham2015understanding,papernot2016distillation}, and techniques to analyze the general properties of adversarial inputs~\cite{metricforadv, ilyas2019adversarial}. 
% More recent work has shown that \emph{natural} variants of input data, \eg rotating an image, changing the lighting conditions, \etc can also make a DNN mispredict~\cite{engstrom2019exploring, pei2017deepxplore,tian2017deeptest,zhang2018deeproad}. As the name suggests, these variations may be perceivable by a human but can occur in a real scenario without any active adversary. However, our knowledge of the robustness properties of DNNs \wrt  such natural variants is still limited. The works that aimed to study such robustness in depth focus on spatial transformations, viz., rotation and translation, because the number of natural variants of an original can be infinite. For example, existing works improve a DNN's robustness against these  spatially transformed images using data augmentation~\cite{engstrom2019exploring} and extra regularization term~\cite{trade_alp_spatial}. \cite{geometric_certify} further provides a DNN verification method for spatial transformation. However, we still do not have a clear idea about the robustness properties of DNN against these transformations, for example, in which cases the DNNs are more prone to failure, whether robustness is inherent in the dataset or depends on the model, etc. 

% More recent work has shown that \emph{natural} variants of input data can also make a DNN mispredict~\cite{engstrom2019exploring}. Natural variants are designed to simulate variations in the configuration or context of data capture, such as a change in the camera angle, orientation, zoom-factor, or lighting conditions during image capture, or more broadly, changing the background or ambient conditions of a subject being captured~\cite{pei2017deepxplore,tian2017deeptest,zhang2018deeproad}. However, unlike the substantial body of work on adversarial examples, there is still a limited number of work on the robustness of DNNs with respect to such natural variants. Engstorm et al.~\cite{engstrom2019exploring} studies the fragility of DNN under natural variants based attacks and proposes a simple data augmentation method to improve the DNN’s robustness to these attacks. Recently, \cite{trade_alp_spatial} proposes a way to further improve DNN’s robustness by introducing an extra regularization term as in \cite{TRADES, ALP}. \cite{geometric_certify} provides the first verification method for DNNs to spatial transformation. However, none of the existing work provides an in-depth analysis of the robustness properties of DNN against spatial transformations. To fill this gap, in this paper, we conduct an in-depth study of the robustness properties of DNNs in terms of natural variations. In particular, following previous work \cite{engstrom2019exploring}, we use the spatial transformations of rotation and translation to simulate natural variations and %,  as in [18], 
%To bridge this gap, in this paper, we conduct an in-depth study of different robustness properties of DNNs \wrt rotation and translation. 
% study to the robustness properties under such variations as spatial robustness. 



%Most existing DNN testing literatures evaluate robustness by generating testing instances~\cite{pei2017deepxplore, tian2017deeptest, zhang2018deeproad} or adversarial instances ~\cite{goodfellow2014explaining, carlini2017towards} samples and then estimate the accuracy of the DNN on these generated samples, which reflects the overall robustness of the given DNN under a certain setting. However, these metrics fail to measure the local robustness of a DNN on a data point and its variants. Such local robustness measure can be very useful when a user wants to know if a given DNN can have reliable performance on not only the given data point but also on its variations. Thus, in this paper, we quantify the robustness of a DNN in a vicinity of a given input data point by considering a population of natural variants of the point and measuring the fraction of this population classified correctly by the DNN - a high fraction of correct classifications indicates good robustness and vice versa. We term this measure neighbor accuracy. 




% \begin{figure}[htp!]
% \centering
%     \subfloat[]
%     {\includegraphics[width=0.24\textwidth]{{"experiments/figure/motivation1a"}.pdf}
%     \label{fig:accuracy}
%     }
% ~
%     \subfloat[]
%     {\includegraphics[width=0.24\textwidth]{{"experiments/figure/motivation1b2"}.png}
%     \label{fig:intersection}}
    
% \caption{\textbf{\small{a)~Effect of rotation on the accuracy of two state-of-the-art models for \cifar. b)~Fraction of data mis-predicted by both the models.}}}
% \label{fig:accuracy-intersection}
% \end{figure} 

% %% Motivating example
% Before jumping into our empirical study of these questions, we first provide two motivating examples. Figure~\ref{fig:accuracy} shows that the performance of two different state-of-the-art models on the CIFAR-10 dataset deteriorates even if a small range of rotations are applied to the original data. On the one hand, the models fail to classify an extra of 10\% of data in presence of only 5 degrees rotations. On the other hand, for 40\% of data the models predict correctly in the presence of even 30 degrees rotations. Interestingly, Figure ~\ref{fig:intersection} further shows that $60\% - 75\%$ of the mis-classified data are common between the two models for 5 - 30 degrees rotations. These observations illustrate that the robustness of a DNN can vary a lot for different data points in its input space. Further, the data itself rather than the model architecture used may be one of the main reasons for the observed brittleness of DNNs. A natural question to ask, in light of these findings, is whether these problematic data exhibit any characteristic properties.



% While studying the robustness of a model, most existing studies evaluate the accuracy of a DNN model on naturally or adversarially generated image variants~\cite{pei2017deepxplore, tian2017deeptest, zhang2018deeproad,goodfellow2014explaining, carlini2017towards} and report overall robustness of the model under test. However, not all the input images are equally likely to fail. For example, consider~\Cref{fig:motivation_different_classes}: the bird in Figures (a)-(d) is initially correctly classified by a DNN and then are mispredicted to three different classes under different variations. 
% In contrast, another bird image and its rotated versions, shown in Figure~\ref{fig:motivation_different_classes} (e)-(h), are correctly classified by the same DNN under the same degrees of rotation. 

% The examples of Figure~\ref{fig:motivation_different_classes} illustrate another aspect of a DNN’s robustness properties – the diversity of classes to which variants of a given input image are classified. As shown in Figure~\ref{fig:motivation_different_classes} (a)-(d), a bird image which is originally correctly classified by a DNN, can be confused to three different other classes, under different variations. By contrast, another bird image and its rotated versions, shown in Figure~\ref{fig:motivation_different_classes} (e)-(h), can be correctly classified by the same DNN. This disparity begs the question: Is the diversity of a model's prediction on an input image correlated with the model's robustness to that input and its variants?



%%% Summary of our findings.
% We seek answers to the above questions and wonder if we can use our observations to identify points of poor robustness efficiently. To this end, we conduct an empirical analysis of the robustness properties of three popular DNN architectures (to natural variations) across three well-known object recognition datasets, \ie, a total of nine DNN-dataset combinations. Our findings reveal that, for each of the DNNs, the neighbor accuracy can range from 0\% to 100\%, as a function of the input data point. Interestingly, a significant proportion of these weak points are common across different DNNs for a given dataset, \ie, Intrinsic to the dataset rather than the DNN. Besides, the points with weak robustness, \ie low neighbor accuracy, are concentrated near the class decision boundaries of the DNN in the feature space. Further, we observe that the degree of weakness is strongly correlated with the number of different classes that different variants of a point get classified to – variants of weaker points get misclassified to many different classes. Based on these findings, we develop two techniques that can identify points of poor robustness at runtime, thereby providing a means of, input-specific, real-time feedback about robustness to the end-user.


% %%% Contributions
% In summary, we make the following contributions: 
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Empirical study \& metric:} We conduct an empirical study of robustness properties of DNNs to natural variations, using nine DNN models, spanning three popular image classification datasets. We adopt a metric called neighbor accuracy to quantify the robustness of the DNN for any given point in the DNN input space.
%     \item \textbf{Characterization of robustness:} We identify three key properties to characterize DNN robustness, namely, the distribution of points of weak robustness, the spatial distribution of these weak points in the DNN’s representation space, these weak points across different DNNs on the same dataset, and the diversity in the (incorrect) classifications of natural variants of a data point. Our study reveals interesting findings for these properties.
%     \item \textbf{Real-time robustness feedback:} Drawing on the above properties, we develop two different kinds of analysis, one white-box (\toolWB) and another black-box (\toolBB), to provide input-specific real-time feedback to the end-user on the robustness of DNN in the vicinity of a given input.
% \end{itemize}



==> results.tex <==
%auto-ignore
\section{Data Analysis \& Results}
\label{sec:results}

\input{experiments.tex}

\subsection{RQ1: what are the distribution/characteristics of weak points}
% 
\subsection{RQ2: How accurately we can identify the failure region for norm-based perturbation?}



\subsection{RQ3: How the failure region of a dataset varies across different models?}


\subsection{RQ4: If our technique is valid for other vision tasks?} 





% \subsection{RQ1: How accurately we can identify the failure region?}
% \subsubsection{Sample rate for labeling failure/non-failure regions}

% To choose a reasonable sample rate for labeling, we did a sweeping experiments on a resnet56 model trained on CIFAR-10 dataset with augmentation. We generated all 1519 neighbours for each original test data and test these neighbours on the resnet56 model. We computed the failure rate for each test data and labeled the original data point and its neighbours as failure regions or non-failure regions based on the failure rate of the test data. In the sweeping experiments, we labeled each test data in the same way but using sampled neighbours.
% Figure \ref{fig:sweeping-labeling} shows how the labeling accuracy changes as the sample rate of failure/non-failure regions varies. The unit of sample rate in the graph is part per thousand. When sample rate is 0.1(100 parts per thousand), the labeling accuracy is already as high as 0.98. So we will use 0.1 sample rate to label failure/non-failure regions.

% \begin{figure}[!phtb]
% \centering
% \includegraphics[width=\linewidth]{experiments/figure/test_labeling_sweeping_batch.png}

% \caption{\textbf{\small Sweeping for labeling}}
% \label{fig:sweeping-labeling}
% %\vspace{-0.5cm}
% \end{figure}

% \subsubsection{Sample rate for training failure/non-failure regions}

% The training data used in training the surrogate model are the neighbours of original training data in the feature space of original model. It is not either scailable or necessary to train with all the neighbours. To decide how many neighbours used in training, we did a sweeping experiments on a resnet56 model trained on CIFAR-10 dataset with augmentation. We trained a surrogate model with sampled different number of neighbours of original training data and tested the model on all the neighbours of all the test data.
% Figure \ref{fig:sweeping-training} shows that we get the highest well f1 score and pillar f1 score when sampled neighbours of each data points is 8. So we will use 8 as sampled number of neighbours of each training data to train the surrogate models.

% \begin{figure}[!phtb]
% \centering
% \includegraphics[width=\linewidth]{experiments/figure/training_sweeping.png}

% \caption{\textbf{\small Sweeping for training}}
% \label{fig:sweeping-training}
% %\vspace{-0.5cm}
% \end{figure}

% \subsubsection{Sample rate for testing failure/non-failure regions} ~\\
% We did a sweeping experiments in testing a surrogate model trained with 10 sampled neighbours for each training data. We used different sample rate of neighbours of testing data to test the model.
% Table \ref{tab:sample_testing} shows that using 0.01 sample rate can give the same accuracy as using all data(1.0 sample rate). So we will use 0.01 sample rate to test the surrogate models.

% \begin{table}[!phtb]
% \centering
% \scriptsize
% \caption{\textbf{\small Sweeping for testing}}
% \label{tab:sample_testing}
% \begin{tabular}{l|cccccccccc}
% %\begin{tabular}{l|l|rrrrrr}
% \toprule
% sample rate & 0.01 & 0.02 & 0.03 & 0.04 & 0.05 &1.0\\
% \midrule
% non-failure regions f1 & 0.83 & 0.83 & 0.83 & 0.83 & 0.83 & 0.83 \\
% \midrule
% failure regions f1 & 0.64 & 0.64 & 0.64 & 0.64 & 0.64 & 0.64 \\
% \bottomrule
% \end{tabular}

% \end{table}

% \subsubsection{Accuracy on CIFAR-10 dataset}

% \begin{table}[!phtb]
% \centering
% \scriptsize
% \caption{\textbf{\small Accuracy of ResNet56 model on CIFAR-10}}
% \label{tab:sample_testing}
% \begin{tabular}{l|cccc}
% %\begin{tabular}{l|l|rrrrrr}
% \toprule
%  & precision & recall & f1-score & support\\
% \midrule
% non-failure regions f1 & 0.82 & 0.84 & 0.83 & 10142363 \\
% \midrule
% failure regions f1 & 0.66 & 0.64 & 0.65 & 5047637 \\
% \bottomrule
% \end{tabular}

% \end{table}

==> rq.tex <==
%auto-ignore
\section{Research Questions}
\label{sec:res_ques}

We address the following research questions in this paper:

%\RQ{1}{How are the robustness of data points in a dataset distributed on a well trained model? Is the robustness of data points dependent on models or training data?}
\RQ{1}{\rqa}
%First,  we explore the distribution of spatial robustness across different data points of a dataset with respect to a well-trained model. 
%To quantify the robustness of a data point, here we %we adopt a measure called {\em neighbor accuracy} and 
Here we evaluate neighbor accuracy for each data point of a dataset. We conduct these experiments in nine settings (three datasets evaluated on three models). We further explore if such robustness %of the data points 
is inherent to the data (a weak data point is weak across multiple models) or dependent on models by comparing the neighbor accuracy of each point across different models. 
We conclude: 

\begin{result}
%While a majority of the data points of every data set tend to be robust, 
\edited{Around $314,028$ (46\%) data points of the whole data set are weak(total 687,867, 3 times total dataset because of 3 models)}, with neighbor accuracy $<0.75$. Robustness seems to be an intrinsic property of most points and does not vary across models. %\todo{seems? Some data points' neighbour accuracy may depends on models}
%, a non-trivial number ($21,753$, i.e., around 3\%) of points' robustness  vary across models. 
%While the robustness seems to be an intrinsic property of most data points, a non-trivial number ($21,753$, i.e., around 3\%) of points' robustness  vary across models. 
\end{result}


% \begin{result}
% Data points of every dataset have varying degrees of robustness -- while a majority of the data points tend to be robust with high neighbor accuracy, 19.5\% of training data points and 20.3\% of testing data points have very low neighbor accuracy($<$ 0.5) making them non-robust under spatial transformations. Moreover, while the robustness seems to be an intrinsic property of the data, \ie a non-robust data point is non-robust across multiple models, for around 3.2\% (average across all settings, with a change in neighbor accuracy larger than 0.5) of the data points, the degree of robustness is model dependent.
% \end{result}

%In the first RQ, we explore the distribution of robustness of data on a well trained model. To quantify robustness of a data point, we adopt a measure called ``neighbor accuracy". We draw histograms to show how data points are distributed with respect to neighbor accuracy on three datasets. We also explore if the robustness of each data point is inherent or dependent on models by drawing histograms of the change of the same data point's neighbor accuracy across models.


%\RS{1}{Every dataset has data points of different levels of robustness in terms of neighbor accuracy. Most data points tend to have high neighbor accuracy while a non-trivial portion of data points have low neighbor accuracy. Most data points have similar neighbor accuracy across different models. A small portion of data points' neighbor accuracy, however, are dependent on the models.}


With such %Given that there is a 
significant number of weak points, now we question:

\RQ{2}{\rqb}%{What are the characteristics of the non-robust points?}
We  investigate how a DNN interprets robust vs.~non-robust points by examining DNN's feature representations through visualization  (t-SNE~\cite{vanDerMaaten2008} plot).  For each weak point, we further check whether its neighbors are misclassified to single or multiple incorrect classes, which is quantified using a {\em diversity} score.  

% Here we investigate whether non-robust data points have different characteristics compared to robust data points . 
% We approach this question from two directions. First, we study the spatial distribution of non-robust points in a DNN's representation space by plotting t-SNE\cite{vanDerMaaten2008} graphs of data points of different neighbor accuracy, for all three datasets. We also quantitatively evaluate the correlation between a data point's distance to its class center and its neighbor accuracy. Second, we explore if a model will produce dramatically different predictions on different variants of non-robust data point and not for variants of robust points. To this end we investigate a possible correlation between a data point's neighbor accuracy and the number of different classes to which variants (obtained through spatial transformations) of that point can be classified by the DNN.

\begin{result}
A weak data point tends to have a larger distance from its class's center in the representation space. The weaker a point is, its neighbors are likely to be mis-classified to more diverse classes.
%its neighbours are more likely to be mis-predicted to a more diverse set of classes. 
\end{result}

Next, we investigate how we can leverage these characteristics to identify the weak points automatically. To this end, we build two classifiers assuming white-box and black-box access to the model under test.
%In particular, we question:
%design an analysis or a classifier to  identify the non-robust points

%how to leverage these characteristics to identify the non-robust points automatically.

%\RQ{3}{Can we use an analysis or a classifier to automatically identify the non-robust points?}
\RQ{3}{\rqc}
 Leveraging our findings that weak points tend to be on the decision boundary of a class in the DNN's feature space (see RQ2a), we build a classifier \toolWB\ to identify these points. The classifier is a 4-layer fully connected NN, which takes the feature vectors as input and outputs robust vs.~weak points. Note that, \toolWB assumes a white-box setting where it has access to the original model's internal feature representation. 
%In RQ2, we find that the non-robust data points have different characteristics compared with robust data points. In this RQ, we explore if we can accurately identify non-robust points leveraging the different characteristic these points have. We propose a method called \toolWB\ to identify non-robust points. In particular, we train a 4-layer fully connected NN on the feature vector of training data points with their neighbor accuracy as the detector and evaluate its classification accuracy in terms of precision, recall, the number of true positives, and the number of false positives. We also conduct an ablation study on hyper-parameter selection and explore the trade-off between precision and recall of the trained detector.

\begin{result}
\toolWB can identify non-robust points with f1 score up to 91.4\%, with an average of 76.9\%, at neighbor accuracy < 0.75.
\end{result}


\RQ{4}{\rqd}
%when we only have oracle access to the given DNN classifier?}
%In RQ3, we present a white-box way to identify non-robust points automatically. In this RQ, we explore if we can still identify non-robust points even with only black-box access to the original classifier. In particular, we leverage our observation in RQ2 on the high correlation between a model's predictions' diversity and neighbor accuracy, and propose a method that reports data with high diversity score as top candidates for non-robust points. We evaluate our proposed method, \toolBB, by drawing an auc-roc curve under each setting to evaluate the performance of our method at every diversity score threshold and also report precision, recall, the number of true positives, and the number of false positives at a certain threshold chosen using the training data. 
Leveraging our observation (see RQ2b) on the high correlation between a model's output diversity and neighbor accuracy, we propose a method, \toolBB that reports data with high output diversity scores as potential weak points. Note that \toolBB works in a black-box setting where it only observes models' output without accessing its internals.

\begin{result}
We can identify non-robust points with f1 score up to 99.1\% (on average 96.5\%), respectively, at neighbor accuracy cutoff 0.75, even with only black-box access of the given DNN classifier.
\end{result}

Finally, to check whether these observations are valid in a 
more complicated setting, we ask: %applied our method to another application?

\RQ{5}{\rqe}
\edited{We apply \toolWB into identifying the weak points for a self-driving car application, which uses a regression model instead of a classification model. We further add rain and fog on the original images to generate the neighbors. This emulates a more natural scenario for the car application, as also studied by earlier work~\cite{tian2017deeptest}.}

\begin{result}
\edited{\toolWB can identify weak points with f1 score up to 78.9\%, with an average of 58.2\%, respectively, at neighbor accuracy cutoff 0.75.}
\end{result}

==> rq1.tex <==
%auto-ignore


\section{Results}
\label{sec:result}

In this section, we elaborate on our results.
The first four RQs are based on the controlled study, where we spatially transformed the images with varying degrees of spatial transformations  for analyzing image classification models. 
RQ1 and RQ2 present our empirical findings on the different characteristics of local robustness. 
In RQ3 and RQ4, we evaluate \toolWB and \toolBB in identifying the weak points.
In RQ5, we evaluate the generalizability of our method by applying \toolWB in a regression task for self-driving cars under more complex transformations.

\smallskip
\RQ{1}{\rqa}
\label{sec:rq1}

\noindent
We first explore the distribution of spatial robustness %, measured using  {\em neighbor accuracy}, 
of the studied data sets w.r.t. three well-trained models.
%We measure spatial robustness in terms of {\em neighbor accuracy}. 
In particular, we explore the variations of spatial robustness: a) across different data points of a given model, b) across different models of a given data point.

% \renewcommand{\theenumi}{\alph{enumi}}
% %\begin{itemize}
% \begin{enumerate}[label=\alph*),leftmargin=\parindent] 
%     \item  across different data points of a given model. 
%     \item across different models of a given data point.
%     %\item Given a well trained model, how spatial robustness changes across different data points?
%   % \item RQ1b. Across different models, does spatial robustness of a given point vary?
%   % \item Given a data point, how spatial robustness changes across different models?

% \end{enumerate}

\begin{figure}[!htpb]
\centering
       \includegraphics[width=0.6\linewidth]{experiments/rq1/cifar10_combine5_2.pdf}
  %\caption{\small Train data neighbor accuracy}
\caption{\textbf{\small Histogram of neighbor accuracy for \cifar}}
\label{fig:histogram1}
% \vspace{-0.3cm}
\end{figure}

% \begin{figure}[!htpb]
% \centering
      
%   \includegraphics[width=\linewidth]{experiments/rq1/cifar10_2_withoutlastbin.pdf}
%   %\caption{\small Train data neighbor accuracy}
% \caption{\textbf{\small Histogram of neighbor accuracy for \cifar~without last bin}}
% \label{fig:histogram2}
% %\vspace{-0.3cm}
% \end{figure}

%\RQ{1a}{How neighbor accuracy of data points in a dataset is distributed on a well trained model?}
\medskip
\RQA{1a}{Given a well trained model, how spatial robustness changes across different data points?} 
%Previous work tends to focus on an aggregated spatial robust accuracy measure, i.e., evaluating the overall accuracy of a model under different transformations \cite{engstrom2019exploring}. 
Here, we explore the spatial robustness of each point as captured by its neighbor accuracy. To have a fine-granular understanding, we draw the distribution of neighbor accuracy of data points in both training set and testing set of \cifar\ when using \vgg, \resnet\, and \wrn\  models, respectively, as shown in Figure \ref{fig:histogram1}. The histograms show that for all these models, the neighbor accuracy vary widely across data points\textemdash most of the data points have very high neighbor accuracy, %(60\% of training data and 58\% testing data have neighbor accuracy $>=$0.75),  
there is a non-trivial number of points having relatively low neighbor accuracy (40\% of training data and 42\% of testing data have neighbor accuracy $<$0.75). 
%For example, we see for \vgg\ model, 17.8\% of the testing data points have less than 50\% neighbor accuracy; 
We call such low accuracy points to be  {\em weak} or {non-robust points}. 
Similarly, for neighbor accuracy $<$0.50, around 16\%  of training data and 20\% of testing data turned out to be weak. 
These points degrade the aggregated spatial robustness of the model. The same finding also holds for the other two datasets. 


The distribution of neighbor accuracy on the training data (not shown in Figure \ref{fig:histogram1}) looks similar to that for the testing data. Table \ref{tab:correlation2} 
further shows that correlation of the number of points in each neighbor accuracy bin between training and testing data is very strong (0.999 to 0.944) with statistical significance ($p < 0.05$). %Thus, a strong correlation exists between the training data and testing data in terms of neighbor accuracy. 
%Even among less robust points (neighbor accuracy $<$ 1) this observation is true. 
%if we do not consider perfectly robust points (as spatial robustness is imbalanced), we see high correlation between training and testing data (the last  row of  the table). 
Such strong correlation is perhaps not surprising, as training and testing data are taken from the same data distributions.

{
\begin{table}[htpb]
\setlength{\tabcolsep}{2pt}
\centering
\footnotesize
\vspace{-3mm}
\caption{\small{\textbf{Correlation of spatial robustness (\ie the number of points per neighbor accuracy bin) between training and testing data}}}
\label{tab:correlation2}
\begin{tabular}{l|l|l|l|l|l|l|l|l|l}
\toprule
Dataset  & \multicolumn{3}{c|}{\cifar} & \multicolumn{3}{c|}{\svhn} & \multicolumn{3}{c}{\fmnist} \\
\midrule
Model  & \vgg & \resnet & \wrn & \vgg & \resnet & \wrn & \vgg & \resnet & \wrn \\

\midrule
spearman &  0.944          & 0.979         &    0.970       &     0.977      &     0.997      &    0.998       &    0.995      &   0.983        &  0.995 \\
pearson  &  0.998          & 0.996         &    0.997       &     0.998      &     0.995      &    0.999       &    0.995      &   0.990        &  0.995  \\ 
%pearson* &  0.990          & 0.965         &  0.973         &    0.963       &    0.960       &   0.964        &  0.916         &   0.879        &   0.921    \\ 
\bottomrule
%\multicolumn{10}{l}{* w/o last bin}
%\vspace{-3mm}
\end{tabular}
\end{table}

% \RS{1c}{Training and testing data tend to have similar neighbor accuracy distribution.}
}

% \RS{1a}{
% A non-trivial number of data points across all the datasets are weak \textemdash around 46\% (at cutoff $<$ 0.75) and 18\%  (at cutoff $<$ 0.50) points, on average, have low neighbor accuracy making them non-robust under spatial transformations. %Moreover, while the robustness seems to be an intrinsic property of the data, i.e., a non-robust data point is non-robust across multiple models, 2\%(average all setting with change smaller than 0.5)  of the data points' robustness is also dependent on the models.
% }

\begin{figure}[!htpb]
%\vspace{-3mm}
\centering
          \includegraphics[width=0.6\linewidth]{experiments/rq1/diff2_2.pdf}
          %\caption{\small Per datapoint neighbor accuracy change}
\caption{\textbf{\small Histogram of per data point neighbor accuracy changes for three datasets from \vgg~ model to \resnet~ model across all the three datasets on testing data. }}
\label{fig:histogram3}
%\vspace{-0.3cm}
% \vspace{-3mm}
\end{figure}

\RQA{1b}{Given a data point, how spatial robustness changes across different models?}
Figure \ref{fig:histogram1} shows that the distribution of neighbor accuracy for a dataset looks similar across different models, indicating robustness may be a property of the dataset itself and may not depend on the underlying model architecture. To dig further, for a given dataset, we divide the neighbor accuracy of all data points into 20 equal-sized bins and compute the Spearman and Pearson correlations of the number of points falling into every bin between any two models.   To reduce the potential bias induced by the large portion of original points having neighbor accuracy higher than 95\%, we also compute the Pearson correlation without them. Table~\ref{tab:correlation1} shows that the correlations are very high between any two models for all the three datasets confirming that the overall robustness distribution of a dataset is very similar across different models.

\begin{table}[htpb]
% \vspace{-3mm}
\setlength{\tabcolsep}{3pt}
\centering
\footnotesize
\caption{\small{\textbf{Correlation between models in number of points per neighbor accuracy bin}}}
\label{tab:correlation1}
%\begin{tabularx}{0.95\columnwidth}{l|l|l|c|c|c}
\begin{tabular}{l|l|l|r|r|r}
\toprule
Dataset  &  Setting & Data & Spearman & Pearson & Pearson \\ 
  &   &  &  &  & (w/o last bin) \\ \midrule
\multirow{6}{*}{\cifar} & \multirow{2}{*}{\vgg\ vs \resnet}& Train &0.980&0.985&0.938 \\ %\cmidrule(l){3-6}
& & Test&0.956&0.980&0.920 \\ \cmidrule(l){2-6} 

& \multirow{2}{*}{\vgg\ vs \wrn}&Train&0.995&0.996&0.986 \\ %\cmidrule(l){3-6}
& &Test&0.977&0.995&0.980 \\ \cmidrule(l){2-6}
& \multirow{2}{*}{\resnet\ vs \wrn}&Train&0.991&0.990&0.980 \\ %\cmidrule(l){3-6}
& &Test&0.989&0.986&0.977 \\ \midrule
\multirow{6}{*}{\svhn} & \multirow{2}{*}{\vgg\ vs \resnet}&Train&0.955&0.978&0.979 \\ %\cmidrule(l){3-6}
& &Test&0.995&0.983&0.995 \\ \cmidrule(l){2-6}
& \multirow{2}{*}{\vgg\ vs \wrn}&Train&0.977&0.979&0.993 \\ %\cmidrule(l){3-6}
& &Test&0.998&0.983&0.994 \\ \cmidrule(l){2-6}
& \multirow{2}{*}{\resnet\ vs \wrn}&Train&0.992&0.986&0.955 \\ %\cmidrule(l){3-6}
& &Test&0.998&0.995&0.981 \\ \midrule
\multirow{6}{*}{\fmnist} & \multirow{2}{*}{\vgg\ vs \resnet}&Train&0.863&0.637&0.969 \\ %\cmidrule(l){3-6}
& &Test&0.890&0.627&0.970 \\ \cmidrule(l){2-6}
& \multirow{2}{*}{\vgg\ vs \wrn}&Train&0.877&0.883&0.986 \\ %\cmidrule(l){3-6}
& &Test&0.893&0.874&0.969 \\ \cmidrule(l){2-6}
& \multirow{2}{*}{\resnet\ vs \wrn}&Train&0.967&0.901&0.965 \\ %\cmidrule(l){3-6}
& &Test&0.979&0.899&0.979 \\ %\cmidrule(l){2-6}
\bottomrule
%\vspace{-3mm}
\end{tabular}
%\end{tabularx}
\end{table}

We further examine the per-point variation of robustness across models by analyzing how neighbor accuracy of each data point varies across models.  Figure \ref{fig:histogram3} shows that the change is minimal:  for \cifar, \fmnist~and \svhn, $60\%$, $76\%$, and $81\%$ of data points have neighbor accuracy change less than $0.2$ across the two models. The other datasets also show similar results. This implies that a large portion of data points' neighbor accuracy is independent of the model selected. 
Note that data points that are non-robust across all the models will not be identified by differential testing techniques as proposed by DeepXplore~\cite{pei2017deepxplore}.


% \RS{1b}{Most data points (75\%) have similar neighbor accuracy, aka robustness,  across different models indicating natural robustness is a property of data than model. }
\smallskip
\RS{1}{A non-trivial number of data points (46\% at neighbor accuracy $<0.75$) of the whole data set are weak. 
Robustness seems to be an intrinsic property of the data points and does not vary across models.
%\ziyuan{only giving a number without percentage seems not to show anything interesting? The whole dataset should be 3 times the whole dataset.}
}















